Universal Novelty Detection Through Adaptive Contrastive Learning

Novelty detection is a critical task for deploying machine learning models in the open world. A crucial property of novelty detection methods is universality, which can be interpreted as generalization across various distributions of training or test data. More precisely, for novelty detection, distribution shifts may occur in the training set or the test set. Shifts in the training set refer to cases where we train a novelty detector on a new dataset and expect strong transferability. Conversely, distribution shifts in the test set indicate the methods' performance when the trained model encounters a shifted test sample. We experimentally show that existing methods falter in maintaining universality, which stems from their rigid inductive biases. Motivated by this, we aim for more generalized techniques that have more adaptable inductive biases. In this context, we leverage the fact that contrastive learning provides an efficient framework to easily switch and adapt to new inductive biases through the proper choice of augmentations in forming the negative pairs. We propose a novel probabilistic auto-negative pair generation method AutoAugOOD, along with contrastive learning, to yield a universal novelty detector method. Our experiments demonstrate the superiority of our method under different distribution shifts in various image benchmark datasets. Notably, our method emerges universality in the lens of adaptability to different setups of novelty detection, including one-class, unlabeled multi-class, and labeled multi-class settings. Code: https://github.com/mojtaba-nafez/UNODE

==> sec/2Preliminaries.tex <==

\section{Preliminaries}

\textbf{Contrastive representation learning} 

Contrastive learning is a self-supervised that aims to learn meaningful data representations by pulling positive pairs together and pushing negative pairs apart in the embedding space. 
Let $f_\theta$ be an encoder network that maps an input $x$ to an embedding $z = g_\phi(f_\theta(x))$, where $g_\phi$ is a projection head. Given an input sample $x$, let $\mathcal{P}_x$ be the set of positive examples and $\mathcal{N}_x$ be the set of negative examples. The contrastive loss function is then:

  

\small
$$
\begin{aligned}
     \ell_{\text{con}}(x, \mathcal{P}_{x}, \mathcal{N}_{x}) = - \frac{1}{|\mathcal{P}_{x}|} \log \frac{ \sum\limits_{x_i \in \mathcal{P}_{x}} \exp(\text{sim}(z(x), z(x_i))}{\sum\limits_{x_j \in \mathcal{P}_{x} \cup \mathcal{N}_{x}} \exp(\text{sim}(z(x), z(x_j))}, \\
\end{aligned}
$$
\normalsize

where \(\text{sim}(a, b) = \frac{a \cdot b}{\|a\| \cdot \|b\|}\) represents the cosine similarity between two vectors \(a\) and \(b\).  finally the contrastive loss for a batch of samples $\mathcal{B}:=\left\{x_i\right\}_{i=1}^B $   will be defined as follows:




\small
$$
\begin{aligned}
    & \mathcal{L}_{\text{con}}(\mathcal{B}) = \\
    & \frac{1}{|\mathcal{B}|} \sum_{i=1}^{|\mathcal{B}|} \ell_{\text{con}}(t_1(x_i), t_2(x_i), \mathcal{N}_{x_i}) + \ell_{\text{con}}(t_2(x_i), t_1(x_i), \mathcal{N}_{x_i}) \\
\end{aligned}
$$
\normalsize




where $t_1, t_2 \sim \mathcal{T}$ are augmentations randomly drawn from a predefined family of augmentations $\mathcal{T}$. Then the positive pair $(t_1(x_i), t_2(x_i))$  and the negative set $\mathcal{N}_{x_i} = \{ t_1(x_j) \}_{x_{j \neq i} \in \mathcal{B}} \cup \{ t_2(x_j) \}_{x_{j \neq i} \in \mathcal{B}}$  are formed for contrastive learning.






\textbf{Hard augmention for contrastive learning}
Novelty detection is challenging due to the lack of labels for inlier data. This makes contrastive learning an attractive self-supervised method for learning meaningful representations, as it does not require labels. Motivated by this, many works have applied contrastive learning to novelty detection. However, since all of the inlier samples share the same semantics and could be considered positive pairs, some works have created negative pairs by applying hard augmentations to in-distribution data.
However, despite improvements from contrastive learning, these methods suffer from poor generalizability across different datasets. For instance, it has been shown that rotation works well as a hard augmentation for negative pair creation, but this technique fails on rotation-invariant datasets like medical images. This limitation calls for adaptive, dynamic negative sampling strategies. The choice of hard augmentations should consider the structure and invariances of the particular inlier data distribution.
\\

% \textbf{Negative sample generation}

% Utilizing negative samples for out-of-distribution (OOD) detection tasks, referred to as outlier exposure, involves training a detector model using random auxiliary datasets of outliers. This technique has been shown to enhance the detector's performance. Although using auxiliary outlier data can improve novelty detection, this technique's performance significantly depends on the diversity and distribution shift of the auxiliary outlier dataset compared to the normal samples. For instance, when using CIFAR-10 as the target dataset, utilizing CIFAR-100 as the auxiliary outlier data leads to 98\% AUROC, but using SVHN only leads to 78\% AUROC (results based on the ADIB paper). This demonstrates that related auxiliary outliers are more useful than unrelated or distant outliers. Motivated by this observation, we propose an adaptive method for negative sample creation. Our approach leverages an automated data augmentation strategy to synthesize hard negative samples directly from the normal data distribution. This provides more useful OOD examples compared to sampling from a distant dataset.\\

% \textbf{Hard augmentations for shifting inliers}
% Recent studies have shown that certain augmentations, referred to as "hard augmentation," can generate new samples that significantly diverge from the original data distribution when applied to in-distribution samples. These augmentations are used during training to synthesize out-of-distribution (OOD) samples and improve model performance. However, the effectiveness of augmentations for distribution shifting varies. For example, rotating an image of a "screw" may still appear in-distribution, while rotating an image of a "car" could push it out-of-distribution. This means that augmentations like rotation may induce distribution shifts for some concepts but not others. To improve the generalization of this technique, there is a need for an adaptive hard augmentation method to generate shifted samples conditioned on normal samples.\\



% \textbf{Contrastive learning for novelty detection.} novelty detection seems to be challangeing due to the lack of labels for inlier data, which make contrastivel learning as  powerful self-seupervised learning method for learning meaning ful reprseantion for ND task. motivated by this many works have utilized constrastive learning to tackle ND task. as mentioned befor applying contrastive learning in naive manner will lead to collapse soultion due to lack of negative pairs and based on the this reason previous works, mostly utilized some hard transformation to creat negative pairs and make contrastilve learning training feasible for OOD detection task. However their negative pair generation strategy suffer from applying fixed and non-adaptive set of transformation which limits their applicablity across various dataset. for instance most of previous works rely on rotaion for negative pair generation which is meaning less in many datasete such as medical imaging where inlier data are rotarion agnostic. 





%  \small
% $$
% \begin{aligned}
%       \mathcal{L}_{\text{con}}(\mathcal{B}) =  
%       \frac{\sum\limits_{i=1}^{|\mathcal{B}|} \ell_{\text{con}}(t_1(x_i), t_2(x_i), \mathcal{N}_{x_i}) + \ell_{\text{con}}(t_2(x_i), t_1(x_i), \mathcal{N}_{x_i})}{|\mathcal{B}|}   
% \end{aligned}
% $$
% \normalsize

%  \textbf{Novelty detection}
 
% The novelty detection (ND) task refers to a setup of outlier detection where inlier samples are assumed to share the same underlying concept. During testing, the model must detect which samples belong to the inlier distribution versus outliers. ND is a demanding undertaking due to the lack of information (e.g. labels) about the inlier distribution and the challenges of defining an objective function for the training phase. Formally, one-class experiments are conducted on a dataset with $N$  classes, treating each class in turn as the inlier and the other $N-1$ classes as out-of-distribution (OOD) samples. This process is repeated for each class, averaging performance across all classes to report the overall OOD detection performance.\\

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/Robust_anomaly_detection.tex <==

\section{Robust Anomaly Detection}

It has been shown that deep learning methods are vulnerable to corruptions and distribution shift. This phenomenon is mostly explored in the image classification task, where classifiers struggle to classify corrupted input data. Corrupted inputs are samples that are created by applying various perturbations to the original dataset. These corruptions are designed to mimic real-world distortions that can occur in images, such as noise and compression artifacts. In the novelty detection task, previous works only experiment on clean datasets and report their results on them. However, similar to other learning domains, ND methods - as our results demonstrate - also suffer from the existence of corrupted data. In this section, we compare the robustness of proposed ND methods on corrupted datasets. Interestingly, our superior results indicate that \ours robustly generalizes across corrupted datasets.++

==> tables/OOD_Score_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{Ablation}
    \setlength{\tabcolsep}{4.6pt} % Adjusting column spacing for compactness
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{l*{4}{c}} 
    \toprule
    \noalign{\smallskip}
    \multicolumn{1}{c}{\diagbox{Dataset}{Score}} & $ S_{\text {bin }}$ & $ S_{\text {sim }}$ & $S_{\text \ours}$  \\
    \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    MNIST& 99.0 & 97.5 & 98.7  \\
    CIFAR10 & 96.7 & 85.4 & 96.6  \\
    MVTecAD & 95.4 & 74.4 & 95.9  \\
    SVHN & 80.7 & 74.3 & 83.3 \\
    FMNIST & 93.8 & 86.8 & 93.5 \\
    HEAD-CT & 82.5 & 84.4 & 84.7 \\
    \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    \end{tabular}
    }
    \label{Table:Ablation}
    
\end{table}

 

==> tables/Unlabled_multi_class.tex <==
\begin{table}[h]
	\resizebox{ \linewidth}{!}{\begin{tabular}{llr*{9}{c}} 
			\hline\noalign{\smallskip}
			
			\multicolumn{1}{c}{In} & \multicolumn{1}{c}{Out} && &\multicolumn{1}{c}{Method}  
			\\ \cmidrule(lr){3-7}  
			
			&& \multirow{2}{*}{CSI}  &\multirow{2}{*}{MSAD}   &\multirow{2}{*}{PANDA}  &\multicolumn{1}{c}{ \ours }\\
					&&\multicolumn{1}{c}{ }&\multicolumn{1}{c}{ }&\multicolumn{1}{c}{ }&\multicolumn{1}{c}{ (Ours) }\\
				
			
			\hline\noalign{\smallskip}
			% capsnet: 1911.08616
			% rest: ARAE 97.5	\_	64.1	73 multirow
			\multirow{4}{*}{CIFAR10} 
			&CIFAR100&x&x&x&x& \\
   
			&SVHN&x&x&x&x& \\
			&MNIST& x&x&x&x& \\
			&FMNIST& x&x&x&x& \\
			&ImageNet30&x&x&x&x&\\
			
			\noalign{\smallskip}\hline\noalign{\smallskip}
			
			\multirow{4}{*}{CIFAR100} 
			&CIFAR10&x&x&x&x&\\
			&SVHN& x&x&x&x& \\
			&MNIST& x&x&x&x& \\
			&FMNIST&x&x&x&x& \\
			&ImageNet30&x&x&x&x& \\
			
			\hline
	\end{tabular}}
	
	\caption{ AUROC (\%) of various anomaly detection methods trained on unlabeled CIFAR-10 and CIFAR-100}
	\label{Table 1:Novelty Detection}
	
\end{table}
